Demonstrating the Merits of Integrating Multipath Signals into 5G LoS-Based Positioning Systems for Navigation in Challenging Environments

Constrained environments, such as indoor and urban settings, present a significant challenge for accurate moving object positioning due to the diminished line-of-sight (LoS)communication with the wireless anchor used for positioning. The 5th generation new radio (5G NR) millimeter wave (mmWave) spectrum promises high multipath resolvability in the time and angle domain, enabling the utilization of multipath signals for such problems rather than mitigating their effects. This paper investigates the benefits of integrating multipath signals into 5G LoS-based positioning systems with onboard motion sensors (OBMS). We provide a comprehensive analysis of the positioning system's performance in various conditions of erroneous 5G measurements and outage scenarios, which offers insights into the system's behavior in challenging environments. To validate our approach, we conducted a road test in downtown Toronto, utilizing actual OBMS measurements gathered from sensors installed in the test vehicle. The results indicate that utilization of multipath signals for wireless positioning operating in multipath-rich environments (e.g. urban and indoor) can bridge 5G LoS signal outages, thus enhancing the reliability and accuracy of the positioning solution. The redundant measurements obtained from the multipath signals can enhance the system's robustness, particularly when low-cost 5G receivers with a limited resolution for angle or range measurements are present. This holds true even when only considering the utilization of single-bounce reflections (SBRs).

==> extras.tex <==
%978-1-7281-6535-6/20/$31.00 ©2020 IEEE

% \IEEEpubid{\begin{minipage}[c]{\textwidth}\ \\[12pt]
% 		\\\\\\\\\\\tabz978-1-7281-6535-6/20/\$31.00 \copyright 2021 IEEE.
% 	\end{minipage}}

% Inertial navigation systems (INS), on the other hand, an autonomous system that is not affected by surrounding environments \cite{Noureldin2013}. However, accumulated accelerometer and gyroscope errorsover time, particularly when a micro-electro-mechanical system (MEMS) sensor is used, lead to significant drifts in the navigation solution \cite{Noureldin2013}. GNSS PPP/INS intergation has been developed to overcome the drawbacks of each individual system. Through the integration, the GNSS PPP is used to constriants INS errors in open sky environment then solely relying on INS positioning during GNSS outages. This strategy would only work if either the outages are short or if the INS equipment is of high quality and thus very costly. To compensate for longer outages, researchers opted to utilize perception based systems such as cameras \cite{Ref5}, LiDARs \cite{Ref6} and radars \cite{Ref7}. Each of these technologies would excel in certain scenarios but are not totally reliable under other conditions. Cameras, for example, require a balanced illumination of the scene \cite{Ref5}, which may not be available in some orientations (e.g., when a camera is facing the sun or reflective glass buildings) and time of day. Cameras and LiDARs' performance would also deteriorate in snowing and raining conditions, and radars suffers from low-resolution scans \cite{Ref5,Ref6,Ref7}.

% Approaching this problem through trilateration, requires an estimation filter that optimizes the intersection between multiple noisy measurements. The most commonly utilized being the Extended Kalman Filter (EKF) in GNSS-trilateration. One drawback of EKF is that it assumes linear state dynamics and observation processes, whereas trilateration is fundamentally a non-linear process \cite{Noureldin2013}. Although state dynamics can be linearized through Taylor series expansion, highly non-linear systems will sacrifice the optimality of state estimation. These limitations are not present in Unscented Kalman Filter (UKF) nor the Particle Filter (PF), however, these estimators are time-exhaustive, thus, not deployed in a real-time framework\cite{Noureldin2013}. 
